Density Functional Theory of Model Systems with the Biaxial Nematic Phase

Present work is a theoretical study on the stability of the thermotropic biaxial nematic liquid crystal phase in model systems. Its main aim is to present the phase diagrams of spatially uniform liquid mesophases and to identify the molecular parameters that influence the stability of the biaxial nematic. The diagrams are obtained by means of the Local Density Functional Theory in low density approximation, and the relation between the molecular parameters of the models and macroscopic properties of the system close to the transition point are obtained by means of bifurcation analysis. We consider three model systems; the so-called L=2 model (the lowest coupling model of the orientational part of pair potential), the biaxial Gay-Berne interaction, and the bent-core system. For the second one, we also briefly investigate the temperature dependence of elastic constants in rod-like regime and in the vicinity of the Landau point and comment on the smectic phases. In every case we take into account rigid molecules. We find that the Landau points acquired from the square root rule for hard biaxial ellipsoids retain its significance, and provide qualitatively correct estimations of Landau points positions for Gay-Berne biaxial ellipsoids. In case of the bent-core model molecules build from uniaxial and biaxial Gay-Berne ellipsoids we find that the dipole-dipole interaction and degree of arms biaxiality change the stability of the biaxial nematic phase.

==> appendices.tex <==
%% The "\appendix" call has already been made in the declaration
%% of the "appendices" environment (see thesis.tex).
\chapter{Pointless extras}
\label{app:Pointless}
Appendixes (or should that be ``appendices''?) make you look really clever, 'cos
it's like you had more clever stuff to say than could be fitted into the main
bit of your thesis. Yeah. So everyone should have at least three of them\dots

\section{Like, duh}
\label{sec:Duh}
Padding? What do you mean?

\section{$y = \alpha x^2$}
\label{sec:EqnTitle}
See, maths in titles automatically goes bold where it should (and check the 
table of contents: it \emph{isn't} bold there!) Check the source: nothing
needs to be specified to make this work. Thanks to Donald Arsenau for the
(very teeny) hack that makes this work.

%% Big appendixes should be split off into separate files, just like chapters
%\input{app-myreallybigappendix}


==> backmatter.tex <==
\begin{colophon}
  This thesis was made in \LaTeXe{} using the ``hepthesis'' class~\cite{hepthesis}.
\end{colophon}

%% You're recommended to use the eprint-aware biblio styles which
%% can be obtained from e.g. www.arxiv.org. The file mythesis.bib
%% is derived from the source using the SPIRES Bibtex service.
\bibliographystyle{h-physrev}
\bibliography{mythesis}

%% I prefer to put these tables here rather than making the
%% front matter seemingly interminable. No-one cares, anyway!
\listoffigures
\listoftables

%% If you have time and interest to generate a (decent) index,
%% then you've clearly spent more time on the write-up than the research :)
%\printindex


==> text.tex <==
 Although the  document class defines a shell document in broad typesetting     
  terms, LaTeX needs additional typesetting instructions to format a document    
   completely. Some of these instructions come from document class options, a     
    collection of formatting instructions that define typesetting in more detail.  
     The options can control body text font size, page orientation, number of text  
      columns, print quality, page size, and many other aspects of document design   
       and typesetting.  
